DiffCollage: Parallel Generation of Large Content with Diffusion Models

We present DiffCollage, a compositional diffusion model that can generate large content by leveraging diffusion models trained on generating pieces of the large content. Our approach is based on a factor graph representation where each factor node represents a portion of the content and a variable node represents their overlap. This representation allows us to aggregate intermediate outputs from diffusion models defined on individual nodes to generate content of arbitrary size and shape in parallel without resorting to an autoregressive generation procedure. We apply DiffCollage to various tasks, including infinite image generation, panorama image generation, and long-duration text-guided motion generation. Extensive experimental results with a comparison to strong autoregressive baselines verify the effectiveness of our approach.

==> sections/rebuttal.tex <==
We thank {\rvst, \rvnd, \rvrd, \rvth} for their valuable comments.
We are glad that reviewers find that DiffCollage is ``\textit{clearly written}'' (\rvst) ``\textit{novel and promising}'' (\rvrd), and has ``\textit{extensive experiments}'' (\rvnd) with ``\textit{very high quality, large, and visually globally consistent}'' samples (\rvth) over ``\textit{a variety of applications}'' (\rvst).



\medskip
{\rvrd}: \textbf{Experiment details:}. We use diffusion models pre-trained in a standard manner on existing datasets~(e.g., motion diffusion models trained on short actions and image diffusion models trained on square images). The training process is independent of the factor graph we employ at test time, as long as the pre-trained model can estimate the marginal scores in the factor graph. This gives us the flexibility to apply the same model to perform sampling with different graphs. For example, we can use the same image score model to generate both long images and 360-degree panoramas, defined by different factor graphs. 
\textbf{Influence of factor graphs on results:} 
For example, a factor graph with too small overlapping factors would produce low-quality results, as shown in the right part of the figure below.

\begin{figure}[h]
    \vspace{-0.2cm}
    \centering
    \setlength{\fboxsep}{0pt}%
    \setlength{\fboxrule}{1pt}%
    {
    \adjincludegraphics[height=2.6cm,trim={0 {.32\height} 0 {.43\height}},clip]
    {figure/rebuttal_img.pdf}
    }
    \vspace{-0.2cm}
\end{figure}
\textbf{More details about factor graphs:} 
We use a linear chain graph for long motion/ image generation.
As shown in the left part of the figure above, to generate a motion with two actions ``A person \textcolor{cRUN}{action1}, then \textcolor{cKICK}{action2}.''. We split it into two short actions as factor nodes, $\vy[f^{(1)}]=$``A person \textcolor{cRUN}{action1}'', $\vy[f^{(2)}]=$``A person \textcolor{cKICK}{action2}'', and a null text token as overlap variable $\vy[2]$. The graph can be extended to longer series of actions in Fig.~8.
The example in Sec. 4.1 and Fig.~3 explain chain graphs for image cases. 
\textbf{Diverse marginal distributions of components:}
We note that marginal distributions of motions conditioned on different text prompts are already very diverse, yet DiffCollage is able to generate coherent long motion. We believe this application is similar to the person generation example given by the reviewer and demonstrates DiffCollage's applicability to scenarios with diverse marginal distributions. 


\medskip
{\rvnd}: \textbf{More details on sampling}: 
We did perform a fully parallel sampling of variables. There are indeed conflicts among overlapped factors initially in the noisy data, but they can be gradually reconciled during the denoising process, resulting in a coherent final image. We will add more discussions on this in the revision. \textbf{Shared model for different factors?} Yes, the model is shared among different factors. 
\textbf{Baseline runtime:} We will clarify it in revision, restricting our claim to methods that generates reasonably smooth images. The Baseline generates patches independently and the resulting image is not consistent at all.
\textbf{Chain vs. cycle graph}. As shown in the left figure, a cycle graph can generate a panorama with smooth transitions between the initial and last image, while a chain graph cannot. 

\medskip
{\rvnd, \rvth:} \textbf{More comparisons:}
We are unable to directly compare our method with NUWA-infinity~(no code), Palette~(no official code, only third-party one), or MaskGIT~(only inference code for an ImageNet checkpoint, not suitable for long image generation).
We compare our method with InfinityGAN using its official codebase and default \href{https://github.com/hubert0527/infinityGAN/blob/main/configs/model/InfinityGAN.yaml}{configuration}. As shown in \cref{tab:prec-rec}, DiffCollage performs much better than InfinityGAN. \href{https://anonymouspaper.gitlab.io/diffcollage/infinitygan.html}{Samples.}
Besides, DiffCollage is more general and versatile than those methods specifically designed for in/out-painting~(\cref{tab:comp}).


\medskip
{\rvth}: \textbf{FID of ALIS:} We follow the \href{https://github.com/universome/alis}{official codebase} to train ALIS and use its \href{https://gist.github.com/universome/3140f74058a48aa56a556b0d9e24e857}{data preprocessing} for all compared methods. 
We notice ALIS is trained in more than 167k filtered images while the authors only release 90k unfiltered images in LHQ. The \href{https://github.com/universome/alis/issues/11}{reproduction issues} have also been observed in the community. 
\textbf{Line 398:} Based on the Grid graph in Fig. 2, variable node 1~(in orange) is only connected with factor nodes A and B, instead of 4 nodes.
\textbf{Stronger baseline for Figure 7:} In the inpainting task, the baseline is already the reconstruction method on square images and is different from the (naive) baseline in previous figures. We will change the name to avoid confusion.
\textbf{Influence of sampling steps on quality:}
Indeed, reduced sampling steps not only decrease information exchanges in DiffCollage but also hurts sampling quality for diffusion models in general. We will add more discussion and results on that in the final version.
\textbf{Precision/recall:} See \cref{tab:prec-rec}, DiffCollage achieves a good trade-off between precision and recall.
\textbf{More samples}: we show more random samples in \href{https://anonymouspaper.gitlab.io/diffcollage/index.html}{this anonymous link}.


\begin{table}[]
    \centering
    \scalebox{0.8}{
        \begin{tabular}{cccc}
            \toprule
             Algo        & Parallel & Generality$^+$ & Versatility$^*$ \\
             \hline
             InfinityGAN        & \CG & \XR & \XR \\
             MaskGIT     & \XR & \XR & \XR \\
             Palette     & \XR & \XR & \XR \\
             Ours        &\CG &\CG &\CG\\
             \bottomrule
        \end{tabular}
        }
    \vspace{0.3cm}
    \caption{Comaprison with suggested works. ($+$) Suggested works are only designed for images and can not be generalized to other data, such as motion. ($*$) DiffCollage can be applied to various tasks without retraining, such as image translation~(Sec 5.2).}
    \label{tab:comp}
    \vspace{-0.3cm}
\end{table}

\begin{table}[h]
    \centering
    \scalebox{0.8}{
    \begin{tabular}{cclcl}
    \toprule
& \multicolumn{1}{l}{FID} & FID+  & \multicolumn{1}{l}{Precision} & Recall  \\
\midrule
\cellcolor{lightgray}ALIS & \cellcolor{lightgray}12.60                   & \cellcolor{lightgray}\textbf{14.27} & \cellcolor{lightgray}\textbf{0.79}                   & \cellcolor{lightgray}0.39 \\
\cellcolor{lightgray} InfinityGAN  & \cellcolor{lightgray}15.71 & \cellcolor{lightgray}36.81 & \cellcolor{lightgray}0.33                   & \cellcolor{lightgray}\textbf{0.51} \\
Replacement              & 6.28                    & 28.94 & 0.44               &    \textbf{0.53}\\
Reconstruction           & 6.28                    & 18.37 & 0.60               &       0.49\\
Ours                     & 6.28                    & \textbf{16.43} & \textbf{0.69}               &  0.49\\
\bottomrule
\end{tabular}
}
    \caption{More quantitative comparisons.}
    \label{tab:prec-rec}
\end{table}
